Safety Constrained Multi-UAV Time Coordination: A Bi-level Control Framework in GPS Denied Environment

Unmanned aerial vehicles (UAVs) suffer from sensor drifts in GPS denied environments, which can cause safety issues. To avoid intolerable sensor drifts while completing the time-critical coordination task for multi-UAV systems, we propose a safety constrained bi-level control framework. The first level is the time-critical coordination level that achieves a consensus of coordination states and provides a virtual target which is a function of the coordination state. The second level is the safety-critical control level that is designed to follow the virtual target while adapting the attacked UAV(s) at a path re-planning level to support resilient state estimation. In particular, the time-critical coordination level framework generates the desired speed and position profile of the virtual target based on the multi-UAV cooperative mission by the proposed consensus protocol algorithm. The safety-critical control level is able to make each UAV follow its assigned path while detecting the attacks, estimating the state resiliently, and driving the UAV(s) outside the effective range of the spoofing device within the escape time. The numerical simulations of a three-UAV system demonstrate the effectiveness of the proposed safety constrained bi-level control framework.

==> z_000_author.tex <==
\author{Wenbin Wan
\footnote{Graduate student, Department of Mechanical Science and Engineering, \textit{wenbinw2@illinois.edu}.},
Hunmin Kim\footnote{Postdoctoral Research Associate, Department of Mechanical Science and Engineering, \textit{hunmin@illinois.edu}},
Yikun Cheng
\footnote{Graduate student, Department of Mechanical Science and Engineering,
\textit{yikun2@illinois.edu}.},
Naira Hovakimyan\footnote{Professor, Department of Mechanical Science and Engineering, \textit{nhovakim@illinois.edu}, AIAA Fellow.}
}
\affil{University of Illinois at Urbana-Champaign, Urbana, IL 61801}
\author{
Petros G. Voulgaris\footnote{Professor, Department of Mechanical Engineering, \textit{pvoulgaris@unr.edu}.}}
\affil{University of Nevada, Reno, NV 89557}
\author{
Lui Sha\footnote{Professor, Department of Computer Science, \textit{lrs@illinois.edu}.}
}
\affil{University of Illinois at Urbana-Champaign, Urbana, IL 61801}


% Yikun Cheng
% \footnote{Graduate student, Department of Mechanical Science and Engineering,
% \textit{yikun2@illinois.edu}.},

==> z_06.tex <==
\appendix
\section*{Appendix}
The current appendix presents the UKF algorithm statement and its brief derivation for partially nonlinear systems with sliding window outputs. 
\subsection{UKF with sliding window outputs} \label{sec append}

Consider the system:
\begin{align}
\begin{split}
    x_{k+1}&= A_kx_{k} + w_k\\
    y_k & =   f(x_k) + v_k,
    \label{eq sukf sys}
\end{split}
\end{align}
where $x_k \in {\mathbb R}^n$ is the state, the
output $y_k \in {\mathbb R}^{m}$ represents the measurement of GPS signal strength.
The noise signals $w_k$ and $v_k$ are assumed to be independent and identically distributed (i.i.d.) Gaussian random variables with zero means and  covariances
${\mathbb E[w_k w_k^\top]=\Sigma}_{w'} \geq 0$
and ${\mathbb E[v_k v_k^\top]=\Sigma}_v >0$.

\emph{Algorithm Derivation.}
\subsubsection{Prediction}
Given the previous state estimate $\hat{x}_{k-1}$ and system model~\eqref{eq sukf sys}, the current state can be predicted as
\begin{align*}
    \hat{x}_{k|k-1} = A_{k-1}\hat{x}_{k-1}.
\end{align*}
Its error covariance matrix is
\begin{align*}
    P_{k|k-1} :&= \mathbb{E}[(x_{k}-\hat{x}_{k|k-1})(x_{k}-\hat{x}_{k|k-1})^\top]\\
    &= A_{k-1}P_{k-1}A_{k-1}^\top + \Sigma_{w'},
\end{align*}
where $P_{k-1}:= \mathbb{E}[(x_{k-1}-\hat{x}_{k-1})(x_{k-1}-\hat{x}_{k-1})^\top]$ is the state estimation error covariance matrix. 

\subsubsection{Sigma Points Generation}
We defined a sigma points array
\begin{align*}
    \mathcal{X}_k := \{ \hat{x}_{k|k-1} \pm (\sqrt{nP_{k|k-1}})_i^\top , i=1,\cdots, n\} ,
\end{align*}where $\sqrt{nP_{k|k-1}}$ is the matrix square root such that $\sqrt{nP_{k|k-1}}^ \top\sqrt{nP_{k|k-1}} =nP_{k|k-1}$, and the matrix operator $(\cdot)_i$ gives the $i^{th}$ row of the matrix.

\subsubsection{Measurement Update}
Given the sliding window size $M$, the nonlinear measurement equation $f(\cdot)$ is used to transform the sigma points into predicted measurement vectors
\begin{align*}
\hat{y}_k^i &= f(\mathcal{X}_k^i)\\
\hat{y}_{k-1}^i &= f(A_{k-1}^{-1}\mathcal{X}_k^i)\\
&\vdots\\
\hat{y}_{k-M+1}^i &= f(A_{k-1}^{-M+1}\mathcal{X}_k^i),
\end{align*}
and we define $\boldsymbol{\hat{y}}^i_k := (\hat{y}^i_k , \hat{y}^i_{k-1}, \cdots, \hat{y}^i_{k-M+1})^\top$.

The approximated mean of the measurements is defined by
\begin{align*}
    \boldsymbol{\bar{y}}_k := \sum_{i=0}^{2n}W_k^i \boldsymbol{\hat{y}}_k^i,
\end{align*}
where $W_k^i$ are the weighting coefficients.


%=====================================================
%====.     algorithm  starts      ====================
%=====================================================
\begin{algorithm}[!t] 
\caption{UKF with sliding window outputs}\label{algo1}
\begin{algorithmic}[1]
%=====================================================
\Statex      \ \ \ \ Prediction 
%=====================================================
\State $\hat{x}_{k|k-1} = A_{k-1}\hat{x}_{k-1}$;
%=====================================================
\State $P_{k|k-1} = A_{k-1}P_{k-1}A_{k-1}^\top + \Sigma_{w'}$;
%=====================================================
% \Statex
\Statex      \ \ \ \ Sigma points generation
\State $\mathcal{X}_k = \{ \hat{x}_{k|k-1} \pm (\sqrt{nP_{k|k-1}})_i^\top \}$, $i\in \{1,\cdots, n\}$;
%=====================================================
\Statex      \ \ \ \ Measurement Update
%=====================================================
\For{$i = 1:2n$}
%=====================================================
\State
\begin{align*}
\boldsymbol{\hat{y}_k^i}=\left[
\begin{array}{c}
\hat{y}_k^i\\
\hat{y}_{k-1}^i\\
\vdots\\
\hat{y}_{k-M+1}^i\\
\end{array}
\right]=
\left[
\begin{array}{c}
f(\mathcal{X}_k^i)\\
f(A_{k-1}^{-1}\mathcal{X}_k^i)\\
\vdots\\
f(A_{k-1}^{-M+1}\mathcal{X}_k^i)\\
\end{array}
\right]
\end{align*}
%=====================================================
\EndFor
%=====================================================
\State $\boldsymbol{\bar{y}}_k = \sum_{i=0}^{2n}W_k^i \boldsymbol{\hat{y}}_k^i$;
\vspace{+1mm}
%=====================================================
\State $\boldsymbol{P}_k^{y}=\sum_{i=0}^{2n}W_k^i(\boldsymbol{\hat{y}}_k^i-\boldsymbol{\bar{y}}_k)(\boldsymbol{\hat{y}}_k^i-\boldsymbol{\bar{y}}_k)^\top + {\boldsymbol{\Sigma}_{v}}$;
\vspace{+1mm}
%=====================================================
\State $\boldsymbol{P}_k^{xy} = \sum_{i=0}^{2n}W_k^i (\mathcal{X}_k^i-\hat{x}_{k|k-1})(\boldsymbol{\hat{y}}_k^i-\boldsymbol{\bar{y}}_k)^\top$;
\vspace{+1mm}
%=====================================================
\State $K_k = \boldsymbol{P}_k^{xy}(\boldsymbol{P}^y_k)^{-1}$
\vspace{+1mm}
%=====================================================
\State $\hat{x}_k=\hat{x}_{k|k-1}+K_k(\boldsymbol{y}_k-\boldsymbol{\bar{y}}_k)$;
\vspace{+1mm}
%=====================================================
\State $P_k = P_{k|k-1} - K_k \boldsymbol{P}_k^y K_k^\top  $
%=====================================================
\end{algorithmic}
\end{algorithm}
%=====================================================
%========.     algorithm  ends     ================
%=====================================================

By taking the measurement noises into account, the estimated covariance of the predicted measurements is given by:
\begin{align*}
    \boldsymbol{P}_k^{y}:=\sum_{i=0}^{2n}W_k^i(\boldsymbol{\hat{y}}_k^i-\boldsymbol{\bar{y}}_k)(\boldsymbol{\hat{y}}_k^i-\boldsymbol{\bar{y}}_k)^\top + {\boldsymbol{\Sigma}_{v}},
\end{align*}
where ${\boldsymbol{\Sigma}_{v}} = \diag\{ \Sigma_{v},\cdots,  \Sigma_{v} \}$ is the diagonal matrix.

The cross covariance between the state prediction and predicted measurements is 
\begin{align*}
    \boldsymbol{P}_k^{xy} = \sum_{i=0}^{2n}W_k^i (\mathcal{X}_k^i-\hat{x}_{k|k-1})(\boldsymbol{\hat{y}}_k^i-\boldsymbol{\bar{y}}_k)^\top ,
\end{align*}
where $\mathcal{X}_k^i$ denotes the $i^{th}$ element in $\mathcal{X}_k$.

The measurement $\boldsymbol{y}_k:=[y_k,\cdots,y_{k-M+1}]^\top$ is used to update the propagated prediction $\hat{x}_{k|k-1}$ as $\hat{x}_k=\hat{x}_{k|k-1}+K_k(\boldsymbol{y}_k-\boldsymbol{\bar{y}}_k)$.


The covariance matrix of the state estimation error is 
\begin{align*}
    P_k = P_{k|k-1} - K_k(\boldsymbol{P}_k^{xy})^\top - \boldsymbol{P}_k^{xy}K_k^\top + K_k \boldsymbol{P}_k^{y} K_k^\top.
\end{align*}
The gain matrix $K_k$ is chosen by minimizing the trace norm of $P_k$; i.e. $\min_{K_k}\trace{(P_k)}$. The solution of the program is given by
\begin{align*}
    K_k = \boldsymbol{P}_k^{xy}(\boldsymbol{P}^y_k)^{-1}.
\end{align*}
Note that the prediction step does not need unscented transformation because the dynamic system~\eqref{eq sukf sys} is linear. 
